On Throughput Maximization of Grant-Free Access with Reliability-Latency Constraints

Enabling autonomous driving and industrial automation with wireless networks poses many challenges, which are typically abstracted through reliability and latency requirements. One of the main contributors to latency in cellular networks is the reservation-based access, which involves lengthy and resource-inefficient signaling exchanges. An alternative is to use grant-free access, in which there is no resource reservation. A handful of recent works investigated how to fulfill reliability and latency requirements with different flavors of grant-free solutions. However, the resource efficiency, i.e., the throughput, has been only the secondary focus. In this work, we formulate the throughput of grant-free access under reliability-latency constraints, when the actual number of arrived users or only the arrival distribution are known. We investigate how these different levels of knowledge about the arrival process influence throughput performance of framed slotted ALOHA with $K$-multipacket reception, for the Poisson and Beta arrivals. We show that the throughput under reliability-latency requirements can be significantly improved for the higher expected load of the access network, if the actual number of arrived users is known. This insight motivates the use of techniques for the estimation of the number of arrived users, as this knowledge is not readily available in grant-free access. We also asses the impact of estimation error, showing that for high reliability-latency requirements the gains in throughput are still considerable.

==> reliability_kmpr.tex <==
\subsubsection{Reliability K-MPR}

The reliability can be calculated as the expected number of successful users versus total amount of users can be given with,

\begin{equation}
r ( \parresource, \latency, \nactiveuserrv ,\mpr) = \left({1-\simprob}\right)^{\nactiveuserrv-1}	\sum_{i=0}^{\mpr-1} \cdot {{\nactiveuserrv-1}\choose{i}} \left(\frac{\simprob}{1-\simprob}\right)^{i},
\label{eq:def_rel_mcsa_mpr2}
\end{equation}

where the proof is given in Appendix \ref{app:2}.

\begin{figure}
	\includegraphics[width = 0.5\textwidth]{function_Rel_kmpr}
	\caption{Reliability of framed slotted ALOHA with varying number of \device s $\nactiveuser$~and the $\mpr$ for K-MPR with $\parresource= 10$ and $\latency = 5$.}
	\label{fig:rel_kmpr}
\end{figure}

There are interesting insights to be obtained from this equation. The most important one is, in order to increase reliability increase \mpr~with low load increasing  and decrease \mpr~with the high load. In between the right choice would depend on the combination of number of \device s and number of resources. An example setting with $\parresource=10$ and $\latency=5$ is plotted in Fig.~\ref{fig:rel_kmpr} with varying $\nactiveuserrv$. Up to $15$ \device s it always make sense to have $\mpr=9$. From $15$ to $55$ \device s the optimal $K$ for higher reliability varies and after $50$ $K=1$ provides a higher reliability.


\subsubsection{Throughput K-MPR}

The expected number of resolved \device s in Eq.~\eqref{eq:expected_succ_perres6} can be used to derived throughput as defined in Eq.~\eqref{eq:T} to show

\begin{equation}
	\throughput(\parresource,\latency,\mpr,\nactiveuserrv) = \frac{\nactiveuserrv}{\parresource\latency} \left({1-\simprob}\right)^{\nactiveuserrv-1}	\sum_{i=0}^{\mpr-1} \cdot {{\nactiveuserrv-1}\choose{i}} \left(\frac{\simprob}{1-\simprob}\right)^{i}.
\end{equation}
which is equal to,
\begin{equation}
\throughput(\parresource,\latency,\mpr,\nactiveuserrv) = \frac{\nactiveuserrv}{\parresource\latency} r ( \parresource, \latency, \nactiveuserrv ,\mpr).
\end{equation}
This equation describes the efficient use of resources and demonstrates the linear relationship between the reliability and throughput even with K-MPR for framed slotted ALOHA. In Fig.~\ref{fig:tpt_kmpr} the throughput is plotted for various $\mpr$ values between $1$ to $9$. Interestingly, the maximum is reached with $\mpr = 8$. This is due to limitation of obtaining integer number of K-MPR channels (reflected with flooring operation) out of $\parresource\latency$ resources which results in some left out resources.

\begin{figure}
	\includegraphics[width = 0.47\textwidth]{function_tpt_kmpr}
	\caption{Throughput of framed slotted ALOHA with varying number of \device s $\nactiveuser$~and the $\mpr$ for K-MPR with $\parresource= 10$ and $\latency = 5$.}
	\label{fig:tpt_kmpr}
\end{figure}

\subsubsection{1-MPR}
